Deep Adversarial Learning on Google Home devices

Smart speakers and voice-based virtual assistants are core components for the success of the IoT paradigm. Unfortunately, they are vulnerable to various privacy threats exploiting machine learning to analyze the generated encrypted traffic. To cope with that, deep adversarial learning approaches can be used to build black-box countermeasures altering the network traffic (e.g., via packet padding) and its statistical information. This letter showcases the inadequacy of such countermeasures against machine learning attacks with a dedicated experimental campaign on a real network dataset. Results indicate the need for a major re-engineering to guarantee the suitable protection of commercially available smart speakers.

==> sec/old/adversarial_setup.tex <==
\section{Adversarial Setup \& Techniques}\label{sec:adversarial-setup-2}

As in previous works \cite{caputo2020fine,su2020you,Shahid2019}, the attacker can only acquire encrypted traffic to compute statistical metrics and analyze them using machine learning techniques.
Such a computation requires using a suitable number of packets grouped using either time spans of length $\Delta t$ or bursts of a fixed size of $N$ packets. Table \ref{tab:features_name_statistical_indicator} lists the set of indicators computed for the experimental activity of this letter.

The goal of the defense techniques is to act on those metrics to lower the attacker's classification accuracy.
In this perspective, this letter exploits three different types of adversarial approaches that aim to lower this classification accuracy. 
Ideally, we would like to reduce the classification accuracy to be as close as possible to a ``coin toss" (i.e., 50\% on a two-class classification problem). 
The three techniques that we present, and that will be described later in \ref{sec:adversarial-techniques-2}, are: \textit{i}) smoothing of features through Savitzky--Golay filter, \textit{ii}) injection of Additive White Gaussian Noise (AWGN) into the features time series and \textit{iii}) ``Realistic Adversarial", a targeted approach to feature degradation that also considers the constraints of the protocols and networks in use.

The first two approaches aim to show the theoretical performances that could be obtained by randomizing, without any constraints, the statistics of the packets and the features derived from them.
The third, instead, represents an approach that takes into account which features can effectively be distorted at the egress of the IoT device (therefore with external hardware such as \textit{anonymization box}) without compromising its operation (e.g., it is possible to add padding to the packets, but it is not possible to randomize the TCP window without disrupting the service completely).

%As in previous works \cite{caputo2020fine,su2020you,Shahid2019}, the attacker can rely only on encrypted traffic.
%In order to gain information about smart speakers, the attacker can compute indicators of encrypted traffic by using two different ``grouping" schemes.
%Specifically, we computed the desired metrics by considering a suitable amount of packets obtained according to the following windowing mechanisms:
%\begin{enumerate*}
%	\item time spans of length $\Delta t$; and %(see Figure \ref{fig:packetsdeltat});
%	\item bursts of a fixed length of $N$ packets.% (see Figure \ref{fig:packetsn}).
%\end{enumerate*} 

%Concerning the statistical indicators that an attacker can obtain from the traffic exchanged between the smart speaker and the cloud, we consider those listed in Table \ref{tab:features_name_statistical_indicator}.
%Each indicator can be modified by a user in order to lower the attacker's classification accuracy.
%In this perspective, In this section we present three different types of adversarial approaches that have the aim to lower this classification accuracy (Table \ref{tab:features_name_statistical_indicator}). 
%Ideally, what we would like to achieve is the reduction of the accuracy to the level of ``coin toss" (e.g. 50\% on a two-class classification problem), even if in reality such adversarial performance is very difficult to obtain using modern algorithms and sufficiently large datasets.
%The three techniques that we present, and that will be described later in \ref{sec:adversarial-techniques-2}, are: \textit{i}) smoothing of features through Savitzky--Golay filter, \textit{ii}) injection of Additive White Gaussian Noise (AWGN) into the features time series and \textit{iii}) "Realistic Adversarial", a targeted approach to feature degradation which also takes into account the constraints of the protocols and networks in use.
%The first two approaches aim to show the theoretical performances that could be obtained by randomizing, without any constraints, the statistics of the packets, and the features derived from them.
%The third, on the other hand, represents an approach that takes into account which features can actually be distorted at the egress of the IoT device (therefore with external hardware such as \textit{anonymization box}) without compromising its operation (e.g. it is possible to add padding to the packets but it is not possible to completely randomize the TCP window without disrupting the service).

\begin{table*}[h]
    \renewcommand\arraystretch{1.35}
    \scriptsize
    \centering
    \begin{tabular}{|l|c||l|c|}
        \hline
        \textbf{Feature Name} &\textbf{Adversarial Technique} & \textbf{Feature Name} &\textbf{Adversarial Technique} \\
        \hline \hline
       
        Number of different IP address (\textit{n\_ip\_unique}) & None &  Number of different TCP/UDP ports (\textit{n\_port\_unique}) & AWGN\\ \hline
        
        Number of TCP packets (\textit{n\_pack\_udp}) & AWGN &  Number of UDP packets (\textit{n\_pack\_udp}) & AWGN \\\hline 
        
        Number of ICMP packets (\textit{n\_pack\_icmp}) & AWGN & \textit{Per-}window Inter packet time (\textit{max\_diff\_time}) & None \\\hline
       

        Average of TCP Window (\textit{mean\_window})  & None & Standard deviation of TCP Window (\textit{std\_window}) & None \\\hline
       
        Average of IPT (\textit{mean\_ipt}) & None & Standard deviation of IPT (\textit{std\_ipt})  & AWGN\\ \hline
        
        Average of packet length (\textit{mean\_len\_pack}) & Const. Padding & Standard Deviation of packet length (\textit{std\_len\_pack}) & Set to Zero\\ \hline

       % \st{Average of TTL (\textit{mean\_ttl})} & \st{AWGN} & \st{Standard Deviation of TTL (\textit{std\_ttl})} & \st{AWGN} \\ \hline
         
    \end{tabular}
    \caption{Name and Acronym of statistical indicator used and the adversarial techniques applied to them}
    \label{tab:features_name_statistical_indicator}
\end{table*}

%%% PARTE RIMOSSA %%%
%\davide{forse questa parte qua lo sposterei nel background, o comunque mi sembra roba già scritta lì?}
%This section, therefore, does not address the adversarial problem from the point of view of the attacker who wants to forge some samples in such a way that they are misclassified by the defender's system. 
%On the contrary, it is the defender (the owner of the Google Home device in this specific case) who tries to engineer and scramble the traffic originating from his IoT devices to put packets or sets of packets in the network that are always sufficiently unrelated to each other and whose statistics are so random that they do not allow the attacker's machine learning models to reach significant accuracy.

\subsection{Adversarial Techniques}\label{sec:adversarial-techniques-2}
The first adversarial technique that we propose uses a Savitzky--Golay filter \cite{savitzky1964smoothing} to smooth all features through a moving window.
%The length of the filter window (win=51 for this problem) determines the number of samples that are taken into consideration: these samples are subsequently approximated by a polynomial of user-defined order. 
The length of the filter window (win=51 for this problem) determines the number of samples taken into consideration, and a polynomial of user-defined order subsequently approximates these samples.
In this specific case, we used different polynomials with a degree of 1, 3, 5, 7, and 9.

%In this specific case, as it can be seen in \figurename\textit{~\ref{fig:on-off-smoothing}} and \textit{\ref{fig:on-noise-smoothing}}, polynomials of degree 1, 3, 5, 7 and 9 have been chosen. 
The second adversarial technique uses Additive White Gaussian Noise (AWGN) -- therefore with zero mean -- whose variance is set proportionally to the variance of the original signal subject to adversarial. 
In this specific case, we multiplied the original variance using values in a range from $0.2$ to $2.0$ in the  \textit{Mic On-Off} and \textit{Mic On-Noise} scenario.
However, in the \textit{utility/media/travel} scenario it was necessary to choose much higher values, i.e., $2$, $8$, $16$, $32$, and $64$.
% In this specific case, multipliers from 0.2 to 2.0 were applied to the original variance in the Mic On-Off and Mic On-Noise classification scenario (\figurename\textit{~\ref{fig:on-off-noise}} and \textit{\ref{fig:on-noise-noise}}), while it was necessary to choose much higher values in the Utility/Media/Travel scenario (as can be see in \figurename\textit{~\ref{fig:time-news-meteo-noise}} the values 2, 8, 16, 32 and 64 have been chosen).

Finally, the last considered technique is called Realistic Adversarial.
This technique tries to reproduce the traffic features that would be obtained from an IoT device that implements adversarial techniques in the real world, by producing its own scrambled network traffic. 
% In this case, the following adversarial techniques were applied:
In this case, we applied two adversarial techniques: the \textit{first} is a  \textbf{constant padding} within the whole time series, which was simulated selecting the maximum value of the mean TCP packet length (\textit{mean\_len\_pack}). 
The standard deviation of the TCP packet length (\textit{std\_len\_pack}) was set to zero to match this operation.
The \textit{second} technique concerns the injection of \textbf{AWGN} in the following features:
\begin{itemize}
  \item \textit{std\_ipt}: to simulate jitter while sending packets;
  \item \textit{n\_pack\_tcp} and \textit{n\_pack\_udp}: to simulate decoy connections and packets between endpoints;
  \item \textit{n\_pack\_icmp}: to simulate decoy ping/traceroute packets between endpoints;
  \item \textit{n\_port\_unique}:, to simulate decoy TCP/UDP packets addressed to random port numbers.
\end{itemize}
Moreover, to match the realistic scenario, we cannot modify the following features: \textit{max\_diff\_time}, \textit{n\_ip\_unique}, \textit{mean\_window} and \textit{std\_window}.
We summarized the applicability of the proposed adversarial techniques to the different traffic features in Table \ref{tab:features_name_statistical_indicator}.

%% OLD
% In this case, the following adversarial techniques were applied:
% \begin{itemize}
% \item Constant padding within the whole time series was simulated selecting the maximum value of the mean TCP packet length (\textit{mean\_len\_pack}); the standard deviation of the TCP packet length (\textit{std\_len\_pack}) was set to zero.
% \item AWGN has been injected into the following features:
% \begin{itemize}
%   \item \textit{std\_ipt}: to simulate jitter while sending packets;
%   \item \textit{n\_pack\_tcp} and \textit{n\_pack\_udp}: to simulate decoy connections and packets between endpoints;
%   %  \item \st{number of UDP packets (\textit{n\_pack\_udp}), to simulate decoy packets between endpoints;}
%   \item \textit{n\_pack\_icmp}: to simulate decoy ping/traceroute packets between endpoints;
%   \item \textit{n\_port\_unique}:, to simulate decoy TCP/UDP packets addressed to random port numbers.
% \end{itemize}
% \end{itemize}
% The total number of packets in the interval (\textit{n\_pack}) was set to the sum of \textit{n\_pack\_tcp}, \textit{n\_pack\_udp} and \textit{n\_pack\_icmp}.
% The features that have been left unmodified are: \textit{max\_diff\_time}, \textit{n\_ip\_unique}, \textit{mean\_window} and \textit{std\_window}.


==> sec/old/experimental_testbed.tex <==
\section{Experimental Testbed}
\label{sec:testbed}
We developed an experimental testbed to prove the effectiveness of privacy threats and the inadequacy of countermeasures applied to network traffic of smart speakers. 
Due to the lack of public and comprehensive datasets containing network traffic of smart speakers, we have also developed an automated framework for generating and collecting the relevant network traffic. In essence, a synthetic talker has been created by using various voice records representing a wide range of speakers (e.g., male and female or with different accents or talking speeds) and it has been used to issue commands to a Google Home Mini smart speaker. Traffic has been captured via an instrumented computer acting as an IEEE 802.11 access point running ad-hoc scripts for {\tt tshark}\footnote{\url{https://www.wireshark.org/docs/man-pages/tshark.html}}. 
To implement the attacker, we used machine learning algorithms provided by the scikit-learn and Fast.ai libraries. We considered the most popular techniques commonly used in the literature, i.e., AdaBoost (AB), Decision Tree (DT), k-Nearest Neighbors (kNN), Random Forest (RF) and Neural Networks (NN) \cite{caputo2020fine,li2007accurate,yang2008p2p}.

%To process the dataset and perform computations, we used a computer with an Intel Core i7-3770 processor, with $16$ GB of RAM running the Ubuntu 16.04 LTS operating system. Obtained traffic traces have been anonymized and made available through Kaggle\footnote{\url{https://www.kaggle.com/smartspeaker/google-home-pcap}}.%\cite{GoogleHomePcapDataset}.

The experimental activities were carried out on an Intel Core i7-3770 computer equipped with $16$ GB of RAM and Ubuntu 16.04 LTS. All the generated traffic traces have been anonymized and made available through Kaggle\footnote{\url{https://www.kaggle.com/smartspeaker/google-home-pcap}}.%\cite{GoogleHomePcapDataset}.



\subsection{Experimental Definition \& Dataset}
%\subsection{Design of the Experiments}
In this letter, we extend the dataset already published in another our work \cite{caputo2020fine}. 
The original dataset was composed by three different rounds of tests, each of them 3 days long.  For the first round of tests, the microphone of the smart speaker was manually set off.
Then, for the second round, the microphone was manually set on and the device put in a quiet condition, i.e., the microphone did not receive any stimuli from the surrounding environment, which was completely without noise or voices.
For the last round of tests, we set the microphone on and we simulated the presence of humans speaking to each other or background noise.
In order to mimic the normal use of smart speakers by users, we extended the original dataset considering three different classes of requests that can be performed, i.e., media, travel, and utility\footnote{\url{https://voicebot.ai/2019/03/12/smart-speaker-owners-agree-that-questions-music-and-weather-are-killer-apps-what-comes-next/}}.
In detail, the experiments consist of three different rounds of tests that last three days of measurements, respectively.
In the first part, we focused on retrieving the network traffic generated to playback multimedia content. For example, we captured traffic when the synthetic talker asked questions like \textit{``What's the latest news?"} or \textit{``Play some music"}.
For the second round, we performed queries related to travels, thus accounting for the interaction with services providing traffic indications or weather forecasts. In this case, we asked questions like \textit{``How is the weather today?"}. Lastly, we performed general queries belonging to the utility category, like \textit{``What's on my agenda today?"} and \textit{``What time is it?"}.
%https://www.italki.com/post/question-281316

We collected $30$ seconds of network inbound and outbound network traffic to have a proper tradeoff between accuracy and size of the data for each query. 
Finally, the entire dataset consists of a 9-day long measurement and contains $2,500$, $400$, and $310$ thousand for each round, respectively.

\textcolor{red}{poi manca una frase che dica che sperimentazione si fa dopo - ovvero il deep adversarial}
%To mimic an average user of smart-speaker-capable services, we considered three different classes of requests that can be performed, i.e., media, travel, and utility\footnote{\url{https://voicebot.ai/2019/03/12/smart-speaker-owners-agree-that-questions-music-and-weather-are-killer-apps-what-comes-next/}}.
%In detail, the experiments consist of three different rounds of tests.
%Since the literature lacks of a precise model describing the behavior of the average user of smart-speaker-capable services, we considered three different classes of requests that can be performed, i.e., media, travel and utility\footnote{\url{https://voicebot.ai/2019/03/12/smart-speaker-owners-agree-that-questions-music-and-weather-are-killer-apps-what-comes-next/}}.
%We performed three different rounds of tests. 
%For the first round of tests, we focused on the retrieval of media or information requiring to playback multimedia contents.
%In the first part, we focused on retrieving the network traffic generated to playback multimedia content. As an example, we captured traffic when the synthetic talker asked questions like \textit{``What\textcolor{red}{'}\st{ i}s the news?"} or \textit{``Play some music"}.
%As an example, we captured traffic when the synthetic talker asked questions like \textit{``What\textcolor{red}{'}\st{ i}s the news?"} or \textit{``Play some music"}.
%Luca: Ma siamo sicuri "What is the news"? Mi suona malissimo in inglese. https://www.italki.com/post/question-281316
%For the second round, we performed queries related to travels, thus accounting for the interaction with services providing traffic indications or weather forecasts. In this case, we asked questions like \textit{``How is the weather today?"}. Lastly, to consider the utility category, we performed general queries like \textit{``What's on my agenda for today?"} and \textit{``What time is it?"}.

%To have a suitable amount of data, each experiment lasted 3 days. Thus, the entire dataset has been generated in a 9-day long measurement campaign. 
%For each query, the network traffic generated by the response has been collected for $30$ seconds, as to have a proper tradeoff between accuracy and size of the data. We collected about $2,500$, $400$, and $310$ thousands of packets for the media, travel and utility category, respectively. 

% We collected, $2,333,499$, $395,826$, and $308,544$ for the media, travel and utility category, respectively.

%Luca: semmai è da dire dopo questa roba. 
% Previous works \cite{su2020you,caputo2020fine} have identified and demonstrated how it is possible to infer human presence inside a building by analyzing the network traffic generated by the smart speaker.
% In this paper, however, before proving the feasibility of a mitigations technique against these attacks, we investigated and analyzed whether it was possible to distinguish which category the query made by the user to the smart speaker belongs to.


% \begin{itemize}
% \item \textbf{Number of TCP, UDP, and ICMP packets.} They allow to quantify the composition of the traffic in terms of observed protocols. %UDP datagrams, for example, indicate the presence of voice information by the QUIC protocol, whereas TCP segments may represent the exchange of additional data such as multimedia.

% \item \textbf{Number of different IP addresses and TCP/UDP ports}. The presence of different endpoints could be used to spot interaction between the smart speaker and the IVA cloud, including actions requiring to contact third-party entities or providers.%, IoT nodes, private datacenters or CDN facilities. 

% \item \textbf{\textit{Per}-window Inter packet time (IPT) or packet count}. It determines how traffic is distributed within the two windows used to group packets described in Figure \ref{fig:groupingnpackets}. 
% %The aggressiveness of the source could be used to reveal user activity or stimuli triggered by a vocal input. 

% \item \textbf{Average value and standard deviation of the TCP window}. 
% Those values describe the behaviour of the flow in term of burstiness and bandwidth usage. Such information could lead to indications about how the IVA and its cloud exchange data. 

% \item \textbf{Average value and standard deviation of the IPT.}
% Similarly to the previous case, they can be used to complete information inferred from the packet rate. The IPT could be used to recognize whether a flow is generated by an application with some real-time constraints. 

% \item \textbf{Average value and standard deviation of the packet length.} They hint the type of the application layer; for instance, small packets can suggest the presence of voice-based activities requiring a low (bounded) packetization delay.

% \item \textbf{Average value and standard deviation of the TTL.} It can be used to mark flows belonging to different portions of the network and possibly indicating that the smart speaker has been activated for a task also requiring the interaction with additional providers or actuators (e.g., IoT nodes). 

% \end{itemize}

%We point out that many indicators are intrinsically ``privacy leaking" as they allow a malicious observer to infer some information about the smart home hosting the device \cite{Apthorpe2017c}. 
%For instance, counting different conversations and the number of protocol data units in a timeframe could reveal the presence of specific IoT nodes or the type of the requested operation, e.g., retrieving a summary of the news. 
%At the same time, considering such values could impact on the performance of the classification framework owing to the exploitation of interactions among the different architectural components, which are difficult to forecast. 






==> sec/old/numerical-results.tex <==
\input{sec/results-subfigures}

\section{Experimental Results}
\label{sec:results}
In this section, we show and discuss the numerical results obtained. 
First, we show the performance and accuracy of machine learning algorithms used to infer the query category. 
Next, we discuss possible mitigations that can be applied by a user to protect their privacy. 
These mitigations will be analyzed using deep adversarial learning.

\textbf{Query Classification.}
%\subsection{Query Classification}\label{sec:query_classification}
The threat model used in this paper is based on the assumption that the attacker is able to acquire large quantities of encrypted network packets from several Google Home devices under his control while also listening for days using a Man-in-the-middle attack. 
With this threat model, it is reasonable to assume that the attacker is able to label the collected traffic with great accuracy.
In our experiment, we assume that the attacker is able to collect 3 days of traffic for each query category (i.e., \textit{media}, \textit{utility} and \textit{travel}), similar to \cite{caputo2020fine}.
% The amount of network traffic collected is
% The threat model used in this paper is based on the assumption that the attacker is able to acquire large quantities of encrypted network packets from several Google Home devices under his control while also listening for days using a Man-in-the-middle attack. 
% With this threat model, it is reasonable to assume that the attacker is able to label the collected traffic with great accuracy and, for this reason, the neural network models he will train will tend to converge towards classification accuracies close to 100\% (see \cite{caputo2020fine} and \figurename~\ref{fig:plain_classification_time_news_meteo_pkts}) and they can therefore be used ``in the wild" with unseen traffic maintaining good results. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{adv-figures/accuracies-for-google-home-v1_3-meteo-news-time-balanced-classification-pkts-1024x768.pdf}
    \caption{\textit{Utility/Media/Travel scenario}: classification accuracy of the different machine learning/deep learning models using unmodified original features.}%, before applying any adversarial techniques to the dataset.}
    \label{fig:plain_classification_time_news_meteo_pkts}
\end{figure}
\figurename~\ref{fig:plain_classification_time_news_meteo_pkts} depicts the accuracy obtained by using several machine learning algorithms to identify the query's category asked by the user.
With a sufficient number of packets within a window, the accuracy of all machine learning models tends towards 100\%.
This behavior would allow the attacker to use his models ``in the wild" with previously unseen traffic maintaining good results. 

%%% INIZIO PARTE RIMOSSA %%%

% \subsection{The Adversarial Setup}
% \label{sec:adversarial-setup}
% \davide{Qua continuare con la discussione dei results sulla parte adversarial, spostarla in una sezione prima?}
% In Section \ref{sec:query_classification} and in other works \cite{caputo2020fine,su2020you,Shahid2019,cheng2017homespy} have been demonstrated how it is possible to infer the state of IoT devices and the presence or not of users inside a building analyzing and applying machine learning algorithms on the encrypted network traffic generated by these devices. 
% To mitigate these privacy issues, in this section we present three different types of adversarial approaches in an attempt to lower the attacker's classification accuracy. 
% Ideally, what we would like to achieve is the reduction of the accuracy to the level of ``coin toss" (e.g. 50\% on a two-class classification problem), even if in reality such adversarial performance is very difficult to obtain using modern algorithms and sufficiently large datasets. 
% The three techniques that we present, and that will be described later in \ref{sec:adversarial-techniques}, are: \textit{i}) smoothing of features through Savitzky--Golay filter, \textit{ii}) injection of Additive White Gaussian Noise (AWGN) into the features time series and \textit{iii}) "Realistic Adversarial", a targeted approach to feature degradation which also takes into account the constraints of the protocols and networks in use.
% The first two approaches aim to show the theoretical performances that could be obtained by randomizing, without any constraints, the statistics of the packets and the features derived from them.
% The third, on the other hand, represents an approach that takes into account which features can actually be distorted at the egress of the IoT device (therefore with external hardware) without compromising its operation (e.g. it is possible to add padding to the packets but it is not possible to completely randomize the TCP window without disrupting the service).

% This section therefore does not address the adversarial problem from the point of view of the attacker who wants to forge some samples in such a way that they are mis-classified by the defender's system. On the contrary, it is the defender (the owner of the Google Home device in this specific case) who tries to engineer and scramble the traffic originating from his IoT devices to put packets or sets of packets in the network that are always sufficiently unrelated to each other and whose statistics are so random that they do not allow the attacker's machine learning models to reach significant accuracy.

% \subsection{Adversarial Techniques}
% \label{sec:adversarial-techniques}
% \davide{spostarla in una sezione prima?}
% The first adversarial technique we propose uses a Savitzky--Golay filter \cite{savitzky1964smoothing} to smooth all features through a moving window.
% The length of the filter window (win=51 for this problem) determines the number of coefficients that are taken into consideration: these coefficients are subsequently approximated by a polynomial of user-defined order. 
% In this specific case, as can be seen in \figurename\textit{~\ref{fig:on-off-smoothing}} and \textit{\ref{fig:on-noise-smoothing}}, polynomials of degree 1, 3, 5, 7 and 9 have been chosen. The second adversarial technique uses simple Additive White Gaussian Noise (AWGN) -- therefore with zero mean -- whose variance is set proportionally to the variance of the original signal subject to adversarial. In this specific case, multipliers from 0.2 to 2.0 were applied to the original variance in the Mic On-Off and Mic On-Noise classification scenario (\figurename\textit{~\ref{fig:on-off-noise}} and \textit{\ref{fig:on-noise-noise}}), while it was necessary to choose much higher values in the Time/News/Meteo scenario (as can be see in \figurename\textit{~\ref{fig:time-news-meteo-noise}} the values 2, 8, 16, 32 and 64 have been chosen). Finally, the last technique we propose is called Realistic Adversarial and tries to reproduce the traffic features that would be obtained from an IoT device that tries to implement adversarial policies, in real world, by producing its own scrambled network traffic. In this case, the following adversarial techniques were applied:
% \begin{itemize}
% \item Constant padding within the whole time series was simulated selecting the maximum value of the mean TCP packet length (mean\_len\_pack); the standard deviation of the TCP packet length (std\_len\_pack) was set to zero.
% \item AWGN has been injected into the following features:
% \begin{itemize}
%   \item standard deviation of inter-packet time (\textit{std\_ipt}), to simulate jitter while sending packets;
%   \item number of TCP packets (\textit{n\_pack\_tcp}), to simulate decoy connections between endpoints;
%   \item number of UDP packets (\textit{n\_pack\_udp}), to simulate decoy packets between endpoints;
%   \item number of ICMP packets (\textit{n\_pack\_icmp}), to simulate decoy ping/traceroute packets between endpoints;
%   \item unique TCP/UDP port numbers (\textit{n\_port\_unique}), to simulate decoy TCP/UDP packets addressed to random port numbers.
% \end{itemize}
% \end{itemize}
% The total number of packages in the interval (\textit{n\_pack}) was set to the sum of \textit{n\_pack\_tcp}, \textit{n\_pack\_udp} and \textit{n\_pack\_icmp}.

% The features that have not been modified are:
% \begin{itemize}
%   \item \textit{max\_diff\_time}, the number of seconds between the timestamp of the first packet and the timestamp of the last packet in the interval;
%   \item \textit{n\_ip\_unique}, the number of unique IPs, both source and destination, captured in the interval;
%   \item \textit{mean\_ipt}, the mean of the inter-packet time over the interval;
%   \item \textit{mean\_window} and \textit{std\_window}, the mean and variance of the TCP window value.
% \end{itemize}

%%% FINE PARTE RIMOSSA E SCRITTA NELLA SEZIONE PRECEDENTE %%


%\subsection{Mitigation Results} \label{discussion}
\textbf{Mitigation Results.} \figurename~\ref{fig:classification_adversarial_mic_on_off_noise_pkts} shows the accuracy of a classifier trained on data subjected to adversarial techniques. 
%The classifier was not pre-trained with the original data, nor was transfer learning performed from previously trained models. 
The classifier was neither pre-trained with the original data nor fed with previously trained models.
The threat model is therefore that of an attacker who tries to train their machine learning models after the adversarial countermeasures have already been deployed and become effective. 

\figurename\textit{~\ref{fig:on-off-smoothing}} to \textit{\ref{fig:on-off-realistic}} show the accuracy obtained in the \textit{Mic On-Off} classification scenario, while \figurename\textit{~\ref{fig:on-noise-smoothing}} to \textit{\ref{fig:on-noise-realistic}} refer to the \textit{Mic On-Noise} scenario. In both scenarios, the trend is similar: the theoretically most effective adversarial technique is polynomial smoothing because it deprives the signal of most of its high frequency components. On the contrary, AWGN injection is less effective as, especially at low variance multiplier values, it leaves much of the signal, and therefore of the information content, intact.

\figurename\textit{~\ref{fig:on-off-realistic}} and \textit{\ref{fig:on-noise-realistic}}, conversely, show the implementation of a realistic adversarial technique which is therefore not able to degrade all the features simultaneously. As can be seen from the accuracy levels maintained (for some sampling intervals $>$ 1250 pkts, higher than 90\%), the neural network model is sufficiently "intelligent" to correctly predict the class using just the few remaining features and ignoring all the others. In this case, higher AWGN intensity does not appear to affect the prediction in any way.

\figurename~\ref{fig:plain_classification_time_news_meteo_pkts} shows the classification accuracy for a neural network model trained on the original data (not subjected to any adversarial technique) of the \textit{Utility/Media/Travel} scenario. With sampling and feature generation intervals higher than 500 pkts, all the algorithms taken into consideration achieve classification accuracy higher than 90\%, with the simpler KNN algorithm always remaining just above this threshold. The accuracy of the neural network model also tends to drop slightly as the interval increases because the number of samples decreases too much for the training "from scratch" of a neural network (at 1500 pkts, the number of samples is just above 300 units for this scenario).
\figurename~\ref{fig:classification_adversarial_time_news_meteo_pkts} shows the classification performance of a new classifier trained on the traffic features from the \textit{Utility/Media/Travel} scenario, already subjected to adversarial techniques. Again, \figurename\textit{~\ref{fig:time-news-meteo-smoothing}} shows how polynomial smoothing techniques are the most efficient when it comes to adversarial, bringing the accuracy of the classifier to around 40\%, very close to the theoretical level of a 33\% random choice of a problem with 3 classes. 
On the contrary, in \figurename\textit{~\ref{fig:time-news-meteo-noise}} it is possible to appreciate how much a strong AWGN is necessary in order to sufficiently degrade the features for this scenario. 
At the intensity levels used in the \textit{Mic-On} and \textit{Mic-Noise} scenarios (\textit{var\_mult}=2.0), the model is practically always above 70\% accuracy with a peak of 80\% with an interval equal to 1000 pkts. To be able to bring the accuracy level to values close to 33\% of the theoretical random choice, it is necessary to inject on the single feature an AWGN with variance multiplier equal to 64 times the original variance of the signal. Finally, \figurename\textit{~\ref{fig:time-news-meteo-realistic}} shows the accuracy obtained from the same neural network architecture trained on degraded features with realistic adversarial. As in \figurename\textit{~\ref{fig:on-off-realistic}} and \textit{\ref{fig:on-noise-realistic}}, the impossibility of degrading all the features at once, leaving some of them intact, preserves enough information for the neural network to learn to correctly infer the three classes of the problem, even with an accuracy of 95\% considering an interval of 1000 pkts, independently from the magnitude of the injected AWGN.




